Diameter and Automorphisms of Gelfand-Tsetlin Polytopes

We determine the diameter of the 1-skeleton and the combinatorial automorphism group of any Gelfand-Tsetlin polytope GT$_{\lambda}$ associated to an integer partition $\lambda.$

==> macaroni.tex <==
I'm keeping this because I am proud of it, in much the same way a 3rd grader is proud of macaroni art -Ben
\begin{gather*}
\lambda_1 \hspace{50pt}
\lambda_2 \hspace{50pt} 
\lambda_3 \hspace{38pt} \ldots \hspace{62pt} 
\lambda_{k-1} \hspace{50pt} 
\lambda_k\\
\rotatebox[origin=c]{-45}{$\leq$} \hspace{20pt} 
\rotatebox[origin=c]{45}{$\leq$} \hspace{25pt} 
\rotatebox[origin=c]{-45}{$\leq$} \hspace{20pt} 
\rotatebox[origin=c]{45}{$\leq$} \hspace{25pt} 
\rotatebox[origin=c]{-45}{$\leq$} \hspace{20pt} \ldots \hspace{50pt} \rotatebox[origin=c]{45}{$\leq$} \hspace{25pt} 
\rotatebox[origin=c]{-45}{$\leq$} \hspace{25pt} 
\rotatebox[origin=c]{45}{$\leq$} \\
x_{1,1} \hspace{40pt}
x_{1,2} \hspace{40pt}
x_{1,3} \hspace{5pt} \ldots \hspace{10pt}
x_{1, k-2} \hspace{45pt}
x_{1, k-1}
\\
\rotatebox[origin=c]{-45}{$\leq$} \hspace{20pt}
\rotatebox[origin=c]{45}{$\leq$} \hspace{20pt}
\rotatebox[origin=c]{-45}{$\leq$} \hspace{20pt}
\rotatebox[origin=c]{45}{$\leq$} \hspace{25pt} \ldots \hspace{35pt}
\rotatebox[origin=c]{-45}{$\leq$} \hspace{20pt}
\rotatebox[origin=c]{45}{$\leq$} \hspace{20pt}
\\
x_{2, 1} \hspace{30pt}
x_{2, 2} \hspace{33pt} \ldots \hspace{42pt}
x_{2, k-2}
\\
\rotatebox[origin=c]{-45}{$\leq$} \hspace{20pt}
\rotatebox[origin=c]{45}{$\leq$} \hspace{40pt} \ldots \hspace{40pt}
\rotatebox[origin=c]{45}{$\leq$}
\\
x_{3, 1} \hspace{47pt} \ldots \hspace{8pt}
x_{3, k-3}
\\
\rotatebox[origin=c]{-45}{$\leq$} \hspace{50pt}
\rotatebox[origin=c]{45}{$\leq$}
\\
\rotatebox[origin=c]{-45}{$\ldots$} \hspace{15pt}
\rotatebox[origin=c]{45}{$\ldots$}
\\
x_{k-1, 1}
\end{gather*}
